User-Space Emulation Framework for Domain-Specific SoC Design

In this work, we propose a portable, Linux-based emulation framework to provide an ecosystem for hardware-software co-design of Domain-specific SoCs (DSSoCs) and enable their rapid evaluation during the pre-silicon design phase. This framework holistically targets three key challenges of DSSoC design: accelerator integration, resource management, and application development. We address these challenges via a flexible and lightweight user-space runtime environment that enables easy integration of new accelerators, scheduling heuristics, and user applications, and we illustrate the utility of each through various case studies. With signal processing (WiFi and RADAR) as the target domain, we use our framework to evaluate the performance of various dynamic workloads on hypothetical DSSoC hardware configurations composed of mixtures of CPU cores and FFT accelerators using a Zynq UltraScale+TM MPSoC. We show the portability of this framework by conducting a similar study on an Odroid platform composed of big.LITTLE ARM clusters. Finally, we introduce a prototype compilation toolchain that enables automatic mapping of unlabeled C code to DSSoC platforms. Taken together, this environment offers a unique ecosystem to rapidly perform functional verification and obtain performance and utilization estimates that help accelerate convergence towards a final DSSoC design.

==> input_sections/experimental_results.tex <==


%the custom hardware accelerators along with  radar emulation environment by mapping different tasks to cthe FPGA and CPUs on different hardware configurations.





==> input_sections/future_work.tex <==
Currently we have to annotate applications (identify kernels) using user input. In future we will automate the flow of kernel identification, and annotating. 

==> input_sections/scheduler_architecture.tex <==

\subsection {Scheduler Integration}


Give supported algorithms
How testbed is used
And then explain how a new scheduler would be integrated
